MNL-Bandit: A Dynamic Learning Approach to Assortment Selection

We consider a dynamic assortment selection problem, where in every round the retailer offers a subset (assortment) of $N$ substitutable products to a consumer, who selects one of these products according to a multinomial logit (MNL) choice model. The retailer observes this choice and the objective is to dynamically learn the model parameters, while optimizing cumulative revenues over a selling horizon of length $T$. We refer to this exploration-exploitation formulation as the MNL-Bandit problem. Existing methods for this problem follow an "explore-then-exploit" approach, which estimate parameters to a desired accuracy and then, treating these estimates as if they are the correct parameter values, offers the optimal assortment based on these estimates. These approaches require certain a priori knowledge of "separability", determined by the true parameters of the underlying MNL model, and this in turn is critical in determining the length of the exploration period. (Separability refers to the distinguishability of the true optimal assortment from the other sub-optimal alternatives.) In this paper, we give an efficient algorithm that simultaneously explores and exploits, achieving performance independent of the underlying parameters. The algorithm can be implemented in a fully online manner, without knowledge of the horizon length $T$. Furthermore, the algorithm is adaptive in the sense that its performance is near-optimal in both the "well separated" case, as well as the general parameter setting where this separation need not hold.

==> reg1.tex <==
\subsection{Proof Outline}\label{proof_outline_thm1}
In this section, we provide an outline of different steps in proving Theorem~\ref{main_result}. 

\vspace{2mm}
\medskip \noindent{\bf Confidence Intervals.} The first step in our regret analysis is to prove the following two properties of the estimates $v^{UCB}_{i,\ell}$ computed as in \eqref{def:vUCB} for each product $i$. Intuitively, these properties establish $v^{UCB}_{i,\ell}$ as upper confidence bounds converging to actual parameters $v_i$, akin to the upper confidence bounds used in the UCB algorithm for MAB \cite{auer}. Specifically,  we show that $v_i$ is bounded by $v_{i,\ell}^{\sf UCB}$ with high probability. Next, we show that as a product is offered more and more, the estimates $v^{\sf UCB}_{i,\ell}$ converge to the true value with high probability. We provide the precise statements for the above mentioned properties in Lemma \ref{lem:UCBv}. These properties follow from an observation that is conceptually equivalent to the IIA (Independence of Irrelevant Alternatives) property of MNL. This observation  shows that in each epoch $\tau$, $\hat{v}_{i,\tau}$ (the number of purchases of product $i$) provides an independent unbiased estimates of $v_i$. Intuitively, $\hat{v}_{i,\tau}$ is the ratio of probabilities of purchasing product $i$ to preferring product $0$ (no-purchase), which is independent of $S_\tau$. This also explains why we choose to offer $S_\tau$ repeatedly until no-purchase occurs. Given these unbiased i.i.d. estimates from every epoch $\tau$ before $\ell$, we apply a multiplicative Chernoff-Hoeffding bound to prove concentration of $\bar{v}_{i,\ell}$. %Then, the above properties follow from definition of $v^{\sf UCB}_{i,\ell}$.

\medskip \noindent{\bf Correctness of Optimistic Assortment.} The product demand estimates $v^{\sf UCB}_{i,\ell-1}$ were used in \eqref{def:RtildeS} to  define expected revenue estimates $\tilde{R}_\ell(S)$ for every set $S$. In the beginning of every epoch $\ell$, Algorithm \ref{learn_algo} computes the optimistic assortment as $S_\ell = \arg\max_S \tilde{R}_\ell(S)$, and then offers $S_{\ell}$ repeatedly until no-purchase happens.  The next step in the regret analysis is to use above properties of $v^{\sf UCB}_{i,\ell}$ to prove similar, though slightly weaker, properties for the estimates $\tilde{R}_\ell(S)$. First, we show that estimated revenue is an upper confidence bound on the optimal revenue, i.e. $R(S^*)$ is bounded by $\tilde{R}_\ell(S_\ell)$ with high probability. The proof for these properties involves careful use of the structure of MNL model to show that the value of $\textstyle \tilde{R}_\ell(S_\ell) $ is equal to the highest expected revenue achievable by any feasible assortment, among {\it all instances of the problem with parameters in the range} $[0, v^{\sf UCB}_i], i=1,\ldots, n$. Since the actual parameters lie in this range with high probability, we have $\tilde{R}_\ell(S_\ell)$ is at least $R(S^*)$ with high probability. Lemma \ref{lem:UCBS1} provides the precise statement. 

\medskip \noindent{\bf Bounding Regret.} The final part of our analysis is to bound the regret in each epoch. First, we use the above property to bound the loss due to offering the optimistic assortment $S_\ell$. In particular, we show that the loss is bounded by the difference between optimistic estimated revenue, $\tilde{R}_\ell(S_\ell)$, and actual expected revenue, $R(S_\ell)$. We then prove a Lipschitz property of the expected revenue function to bound the difference between optimistic estimate and expected revenues in terms of errors in individual product estimates \mbox{$|v^{\sf UCB}_{i,\ell} - v_i|$}. Finally, we leverage the structure of MNL model and the properties of $v^{UCB}_{i,\ell}$ to bound the regret in each epoch. Lemma \ref{lem:UCBS2} provide the precise statements of above properties. 

Given the above properties, the rest of the proof is relatively straightforward. In rest of this section, we make the above notions precise. Finally, in Appendix \ref{sec:completeProof}, we utilize these properties to complete the proof of Theorem \ref{main_result} .




\subsection{$\mathbf{v^{\sf UCB}_{i,\ell}}$: Upper Confidence Bounds }
\label{sec:UCBv}
In this section, we will show that $v^{\sf UCB}_{i,\ell}$ as upper confidence bounds converging to the true parameters $v_i$ from 
above. Specifically, we have the following result. 

\begin{lemma}\label{lem:UCBv}
%\begin{minipage}[t]{\linewidth}
For every $\ell$, we have the following lemmas. 
\begin{enumerate}
\item $v^{\sf UCB}_{i,\ell}\geq v_i$ with probability at least $1-O\left(\frac{1}{\ell}\right)$ for all $i=1,\cdots,N$. 
\item There exists constants $C_1$ and $C_2$ such that \[\hspace{-25mm}\displaystyle v^{\sf UCB}_{i,\ell} - v_i \leq C_1\sqrt{\frac{v_i\log{(\ell+1)}}{T_i(\ell)}} + C_2\frac{\log{(\ell+1)}}{{T}_i(\ell)}\] with probability at least $1-O\left(\frac{1}{\ell}\right)$.
\end{enumerate}
%\end{minipage}
\end{lemma}

\medskip \noindent  
We first establish that the estimates $\hat{v}_{i,\ell}, \ell \leq L$ are unbiased i.i.d estimates of the true parameter $v_i$ for all products. It is not immediately clear a priori if the estimates $\hat{v}_{i,\ell}, \ell \leq L$ are independent.  In our setting, it is possible that the distribution of estimate $\hat{v}_{i,\ell}$ depends on the offered assortment $S_\ell$, which in turn depends on previous estimates. In lemma \ref{moment_generating}, we show that the moment generating of $\hat{v}_{i,\ell}$ only depends on the parameter $v_i$ and not on the offered assortment $S_\ell$, there by establishing that estimates are identically and independently distributed.  Using the moment generating function, we show that $\hat{v}_{i,\ell}$ is a geometric random variable with mean $v_i$, i.e., $E(\hat{v}_{i,\ell}) = v_i$. We will use this observation and extend the multiplicative Chernoff-Hoeffding bounds discussed in \cite{mitzenmacher} and \cite{Babaioff}  to geometric random variables and derive the result. The  proof is technical and the details are provided in Appendix \ref{sec:UCBv}


\subsection{Optimistic Estimate and Convergence Rates}
\label{sec:UCBS}
In this section, we show that the estimated revenue converges to the optimal expected revenue from 
above. First, we show that the estimated revenue is an upper confidence bound on the optimal revenue. In particular, we have the following result. 
\begin{lemma}\label{lem:UCBS1}
Suppose $S^* \in {\cal S}$ is the assortment with highest expected revenue, and Algorithm \ref{learn_algo} offers $S_\ell \in {\cal S}$ in each epoch $\ell$. Then, for every epoch $\ell \geq 10$, we have 
\[\tilde{R}_\ell(S_\ell) \geq \tilde{R}_\ell(S^*) \geq R(S^*) \; \text{with probability at least}\; \;1-O\left(\frac{1}{\ell}\right).\]
\end{lemma}

\medskip \noindent 
In Lemma \ref{UCB_bound}, we show that the optimal expected revenue is monotone in MNL parameters.   It is important to note that we do not claim that the expected revenue is in general a monotone function, but only value of the expected revenue corresponding to optimal assortment increases with increase in MNL parameters. The result follows from Lemma \ref{lem:UCBv}, where we established that $v^{\sf UCB}_{i,\ell}> v_{i}$ with high probability. We provide the detailed proof in Appendix \ref{sec:UCBSa}.

\medskip \noindent The following result provides the convergence rates of estimate $\tilde{R}_\ell(S_\ell)$ to the optimal expected revenue. 

\begin{lemma}\label{lem:UCBS2}
There exists constants $C_1$ and $C_2$ such that for every $\ell $, we have
\[\textstyle (1+\sum_{j \in S_\ell} v_{j})(\tilde{R}_{\ell}(S_\ell) - R(S_\ell)) \leq C_1\sqrt{\frac{v_i\log{(\ell+1)}}{|\mathcal{T}_i(\ell)|}} + C_2\frac{\log{(\ell+1)}}{|\mathcal{T}_i(\ell)|},\; \text{with probability at least}\;1-O\left(\frac{1}{\ell}\right)\]
\end{lemma}
\medskip \noindent 
In Lemma \ref{lipschitz}, we show that the expected revenue function satisfies a certain kind of Lipschitz condition. Specifically, the difference between estimated, $\tilde{R}_{\ell}(S_\ell)$, and expected revenues,  $R_\ell(S_\ell)$, is bounded by the sum of errors in parameter estimates of the products, $|v^{\sf UCB}_{i,\ell} - v_i|$. This observation in conjunction with the ``optimistic estimates'' property  will let us bound the regret as an aggregated difference between estimated revenues and expected revenues of the offered assortments. Noting that we have already computed convergence rates between the parameter estimates earlier, we can extend them to show that the estimated revenues converge to the optimal revenue from above. We complete the proof in Appendix \ref{sec:UCBSa}.

==> reg4.tex <==

\subsection{Putting it all together: Proof of Theorem \ref{main_result}}
\label{sec:completeProof}
In this section, we formalize the intuition developed in the previous sections and complete the proof of Theorem \ref{main_result}.

Let $S^*$ denote the optimal assortment, our objective is to minimize the {\it regret} defined in \eqref{Regret}, which is same as
%\begin{equation}\label{eq:Regret}
%\begin{aligned}
%Reg(T) &=E\left( \sum_{\ell=1}^L \sum_{t \in \ep{E}_\ell}\left(R(S^*) - R(S_\ell)\right)\right)\\
%\end{aligned}
%\end{equation}
%We start with reformulating the regret  in terms of regret incurred in every epoch. 
%For every epoch $\ell$, let $t_\ell$ denote the time index when the no purchase happened, after which the algorithm progressed to the next epoch. Observe \mbox{Algorithm \ref{learn_algo}} by design, offers an assortment until a no purchase happens. Hence, the conditional expectation of $r_t(S_\ell)$ given $S_\ell$, $E\left(r_{t}(S_\ell) \, \middle | \, S_\ell\right)$ is not the same as $R(S_\ell)$, but is given by
%\begin{equation*}
%E\left(r_{t}(S_\ell) \, \middle | \, S_\ell\right) = 
%\begin{cases}
%E\left(r_{t}(S_\ell) \, \middle | \, S_\ell,\{r_t(S_\ell) \neq 0\}\right) &\quad \text{if $t  \neq t_\ell$} \\
%E\left(r_{t}(S_\ell) \, \middle | \, S_\ell,\{r_t(S_\ell) = 0\}\right) &\quad \text{if $t = t_\ell$} \\
%\end{cases}.
%\end{equation*}
%Hence, we have
%\begin{equation*}
%E\left(r_{t}(S_\ell) \, \middle | \, S_\ell\right) = 
%\begin{cases}
%\displaystyle \frac{1+\sum_{j\in S_\ell} v_j}{\sum_{i\in S_\ell} v_i}R(S_\ell) &\quad \text{if $t < t_\ell$} \\
%0 &\quad \text{if $t = t_\ell$} \\
%\end{cases}.
%\end{equation*} 
\begin{equation}\label{eq:regret_simple}
Reg(T)  = E\left\{\sum_{\ell=1}^L |\ep{E}_\ell| \left(R(S^*) - R(S_\ell)\right)\right\},
\end{equation} 
Note that $L$, $\ep{E}_\ell$ and $S_\ell$ are all random variables and the expectation in equation \eqref{eq:regret_simple} is over these random variables.  Let $V(S_\ell) = \sum_{j\in S_\ell} v_j.$ We have $E(|\ep{E}_\ell|) = 1+V(S_\ell)$ and hence the regret can be reformulated as \begin{equation}\label{eq:ce_regret}
Reg(T) =  E\left\{\sum_{\ell=1}^L \left(1+V(S_\ell)\right)\left(R(S^*)-R(S_\ell)\right)\right\}
\end{equation}
the expectation in equation \eqref{eq:ce_regret} is over the random variables $L$ and $S_\ell$. We now provide the proof sketch for Theorem \ref{main_result} and the complete proof is provided in the full version of the paper.

\proofof{ Theorem \ref{main_result}.}
%, from equation \eqref{eq:regret_simple}, we have that
For sake of brevity, let $\Delta R_\ell {=} (1+V(S_\ell))\left(R(S^*)-R(S_\ell)\right)$, {for all} $\ell = 1,\cdots,L.$
%\begin{equation}\label{eq:simplified_regret}
%\end{equation}
Now the regret can be reformulated as 
\begin{equation}\label{eq:ce_regret_2}
\begin{aligned}
Reg(T) &=  E\left\{\sum_{\ell=1}^L \Delta R_\ell\right\}\\
\end{aligned}
\end{equation}
 Let $T_i$ denote the total number of epochs that offered an assortment containing \mbox{product $i$}. Let $\mathcal{A}_0$ denote the complete set $\Omega$ and for all $\ell =1,\ldots,L$, event $\mathcal{A}_{\ell}$ is given by
\begin{equation*}
\mathcal{A}_{\ell} = \left\{v^{\sf UCB}_{i,\ell} < v_i \;\text{or} \; v^{\sf UCB}_{i,\ell} > v_i + C_1 \sqrt{\frac{v_i}{T_i(\ell)}}\log{(\ell+1)} + C_2\frac{\log^2{(\ell+1)}}{T_i(\ell)} \; \text{for some $i \in S_\ell \cup S^*$}\right\}.
\end{equation*}
Noting that $\mathcal{A}_\ell$ is a rare event and our earlier results on the bounds are true whenever event $\mathcal{A}^c_\ell$ happens, we try to analyze the regret in two scenarios, one when $\ep{A}_\ell$ is true and another when $\ep{A}^c_\ell$ is true. For any event $A$, let $\mathbb{I}(A)$ denote the indicator random variable for the event $A$.  Hence, we have
\begin{equation*}
\begin{aligned}
E\left(\Delta R_\ell\right)= E\left[\Delta R_\ell\cdot\mathbb{I}(\mathcal{A}_{\ell-1}) + \Delta R_\ell\cdot\mathbb{I}(\mathcal{A}^c_{\ell-1})\right]
\end{aligned}
\end{equation*}
Using the fact that $R(S^*)$ and $R(S_\ell)$ are both bounded by one and $V(S_\ell) \leq N$, we have 
\begin{equation*}
\begin{aligned}
E\left(\Delta R_\ell\right) \leq (N+1)\mathcal{P}(\mathcal{A}_{\ell-1}) +E\left[ \Delta R_\ell\cdot\mathbb{I}(\mathcal{A}^c_{\ell-1})\right].
\end{aligned}
\end{equation*}
Whenever $\mathbb{I}(\mathcal{A}^c_{\ell-1}) = 1$, from Lemma \ref{UCB_bound}, we have $\tilde{R}_\ell(S^*) \geq R(S^*)$ and by our algorithm design, we have $\tilde{R}_\ell(S_\ell) \geq \tilde{R}_\ell(S^*)$ for all $\ell \geq 2$. Therefore, it follows that 
\begin{equation*}
E\left\{\Delta R_\ell\right\} \leq (N+1)\mathcal{P}(\mathcal{A}_{\ell-1}) +E\left\{\left[(1+V(S_\ell))(\tilde{R}_\ell(S_\ell) - R(S_\ell))\right]\cdot \mathbb{I}(\mathcal{A}^c_{\ell-1}) \right\}
\end{equation*}
From Lemma \ref{lem:UCBS2}, it follows that
\begin{equation*}
\begin{aligned}
\left[(1+V(S_\ell))(\tilde{R}_\ell(S_\ell) - R(S_\ell))\right]\cdot \mathbb{I}(\mathcal{A}^c_{\ell-1}) \leq \log{(\ell+1)}\sum_{i\in S_\ell}\left(C_1\sqrt{\frac{v_i}{T_i(\ell)}} + \frac{C_2\log{(\ell+1)}}{T_i(\ell)}\right)\;
\end{aligned}
\end{equation*}
Therefore, we have
\begin{equation}\label{eq:stoch_dom}
\begin{aligned}
E\left\{\Delta R_\ell\right\} &\leq (N+1)\mathcal{P}\left(\mathcal{A}_{\ell-1}\right) + C E\left(\log{(\ell+1)}\sum_{i\in S_\ell}\left(\sqrt{\frac{v_i}{T_i(\ell)}} + \frac{\log{(\ell+1)}}{T_i(\ell)}\right)\right)\\
\end{aligned}
\end{equation}
where $C = \max\{C_1,C_2\}$. Combining equations \eqref{eq:ce_regret} and \eqref{eq:stoch_dom}, we have 
\begin{equation*}
Reg(T) \leq E\left\{\sum_{\ell=1}^L \left[(N+1)\mathcal{P}\left(\mathcal{A}_{\ell-1}\right) + C\log{(\ell+1)}\sum_{i\in S_\ell}\left(\sqrt{\frac{v_i}{T_i(\ell)}} + \frac{\log{(\ell+1)}}{T_i(\ell)}\right)\right] \right\}.
\end{equation*}
Therefore, from Lemma \ref{lem:UCBv}, we have
\begin{equation}\label{eq:regret_bound_first_step}
\begin{aligned}
Reg(T)& \leq CE\left\{\sum_{\ell=1}^L \frac{N+1}{\ell} +\sum_{i\in S_\ell}\sqrt{\frac{v_i}{T_i(\ell)}}\log{(\ell+1)} + \sum_{i\in S_\ell}\frac{\log^2{(\ell+1)}}{T_i(\ell)}\right\},\\
& \overset{(a)}{\le} CN+ CN\log^3{T} + (C\log{T})E\left(\sum_{i=1}^n  \sqrt{v_iT_i} \right) \\
& \overset{(b)}{\le} CN + CN\log^3{T} + (C\log{T})\sum_{i=1}^N  \sqrt{v_iE(T_i)}
\end{aligned}
\end{equation}
Inequality (a) follows from the observation that $L \leq T$, $T_i \leq T$, $\displaystyle \sum_{T_i(\ell)=1}^{T_i} \frac{1}{\sqrt{T_i(\ell)}} \leq \sqrt{T_i}$ and $\displaystyle \sum_{T_i(\ell)=1}^{T_i} \frac{1}{{T_i(\ell)}} \leq \log{T_i}$, while Inequality (b) follows from Jensen's inequality. 

 For any realization of $L$, $\ep{E}_\ell$, $T_i$, and $S_\ell$ in Algorithm \ref{learn_algo}, we have the following relation $\sum_{\ell=1}^L n_\ell  \leq T$. Hence, we have $E\left(\sum_{\ell=1}^L n_\ell\right)  \leq T.$
Let $\mathcal{S}$ denote the filtration corresponding to the offered assortments $S_1,\cdots,S_L$, then by law of total expectation, we have, 
\begin{equation*}
\begin{aligned}
E\left(\sum_{\ell=1}^L n_\ell\right) &= E\left\{\sum_{\ell=1}^L E_{\mathcal{S}}\left( n_\ell\right)\right\}= E\left\{\sum_{\ell=1}^L1+\sum_{i\in S_\ell} v_i\right\} \\
&=  E\left\{L+\sum_{i=1}^n  v_i T_i\right\} = E\{L\}+\sum_{i=1}^n  v_i E(T_i).
\end{aligned}
\end{equation*}
Therefore, it follows that  
\begin{equation}\label{eq:conditional_ineq}
\sum v_iE(T_i) \leq T.
\end{equation}
To obtain the worst case upper bound, we maximize the bound in equation \eqref{eq:regret_bound_first_step} subject to the condition \eqref{eq:conditional_ineq} and hence, we have $Reg(T) =   O( \sqrt{NT}  \log{T} + N\log^3{T}).$ \hfill $\Halmos$
